Label-Free Performance Monitoring of Wireless Foundation Models: Error Estimation, Drift Detection, and Estimator Selection in O-RAN

Wireless physical-layer foundation models (WPFMs) are promising channel estimators, but their accuracy under changing conditions cannot be assessed without ground-truth channel state information (CSI). We develop a label-free monitoring framework for WPFM-based channel estimation in Open Radio Access Networks (O-RAN). Comparing reconstructions of held-out pilots with noisy least-squares observations gives a CSI-free estimate of the channel-estimation mean-squared error (MSE). We characterize its bias and finite-sample concentration, derive conditional pairwise estimator-comparison statistics, and bound the monitored-to-deployed error gap. These results support cumulative sum (CUSUM) drift detection and estimator fallback. The selection guarantees concern held-out error, not deployed estimation error or block error rate (BLER). In 3GPP and ray-traced simulations, the detector meets its false-alarm target in 113 of 135 cases with 100 calibration windows, and in 128 (135 with 200 windows) with tail-aware calibration. Fallback improves normalized MSE (NMSE) by 2.4-4.1 dB over a frozen WPFM, but MSE-based selection can yield much higher BLER than linear minimum MSE (LMMSE) estimation. A receiver-aware directional statistic lowers this BLER on a switching schedule from 0.33-0.39 to 0.19-0.20 over five runs, still above LMMSE (0.16-0.17). Test-time training increased NMSE after 200 steps, and the slower adaptation loops added little to real-time fallback.

==> figs/cmapstyle.tex <==
%
\pgfplotsset{cmapax/.style={width=3.0cm, height=2.3cm, scale only axis, enlargelimits=false, axis on top,
  xmin=-0.5, xmax=12.5, ymin=-0.5, ymax=9.5, y dir=reverse, tick style={draw=none},
  xtick={0,2,4,6,8,10,12}, xticklabels={$-10$,$-5$,0,5,10,15,20}, xticklabel style={font=\tiny, inner sep=1pt},
  ytick={0,...,9}, yticklabels={}, title style={font=\scriptsize, yshift=-1.0ex}, xlabel={SNR [dB]},
  xlabel style={font=\tiny, yshift=0.9ex},
  extra y ticks={1.5,3.5}, extra y tick labels={}, extra y tick style={grid=major, major grid style={black, line width=0.5pt}},
  extra x ticks={1.5}, extra x tick labels={}, extra x tick style={grid=major, major grid style={black, densely dashed, line width=0.5pt}}},
  divmap/.style={colormap={div}{rgb255=(33,102,172) rgb255=(103,169,207) rgb255=(209,229,240) rgb255=(247,247,247)
  rgb255=(253,219,199) rgb255=(239,138,98) rgb255=(178,24,43)}, point meta min=-15, point meta max=15},
  regmap/.style={colormap={reg}{rgb255=(255,255,255) rgb255=(253,219,199) rgb255=(244,165,130) rgb255=(214,96,77)
  rgb255=(178,24,43) rgb255=(103,0,31)}, point meta min=0, point meta max=6},
  alarmmap/.style={colormap/viridis, point meta min=0, point meta max=1},
  kapmap/.style={colormap={kap}{rgb255=(247,247,247) rgb255=(254,224,182) rgb255=(253,184,99) rgb255=(224,130,20)
  rgb255=(179,88,6) rgb255=(127,59,8)}, point meta min=0, point meta max=4}}
\providecommand{\cmapplot}[1]{\addplot[matrix plot*, mesh/cols=13, point meta=explicit] table[x=x, y=y, meta=c] {figs/data/#1};}
\providecommand{\cmapmark}[3]{\addplot[only marks, mark=*, mark size=0.7pt, draw=black, fill=white, line width=0.25pt]
  table[x=x, y=y, restrict expr to domain={\thisrow{#2}}{#3:#3}] {figs/data/#1};}


==> figs/data/v02_cmap_labels.tex <==
%
\def\cmregimes{{CDL-A},{CDL-B},{CDL-D, 50\,ns, 30\,km/h},{TDL-C, 300\,ns, 30\,km/h},{CDL-E},{CDL-A, 300\,ns},{CDL-A, 60\,km/h},{CDL-A, 120\,km/h},{TDL-A, corr.},{CDL-C, 300\,ns}}
\def\cmsnrs{$-10$,$-7.5$,$-5$,$-2.5$,0,2.5,5,7.5,10,12.5,15,17.5,20}


==> figs/data/v02_scorecard_labels.tex <==
%
\def\scoremethods{{LMMSE},{frozen WPFM},{LMMSE, genie stats$^\dagger$},{equal-footprint},{always-on TTT},{periodic retraining},{BLER-trig.\ retraining},{proposed: RT},{proposed: full},{regime oracle$^\dagger$}}
\def\scorephases{{CDL-A},{CDL-C 300\,ns},{CDL-A 60\,km/h},{TDL-A corr.},{CDL-B 200\,ns},{CDL-A},{10\,dB},{0\,dB},{20\,dB},{CDL-A},{blend},{CDL-C},{CDL-A},{ray-traced},{\textbf{worst}}}


==> figs/linkstyle.tex <==
%
%
%
%
\pgfplotsset{linkheat/.style={width=2.75cm, height=2.8cm, scale only axis, enlargelimits=false, axis on top,
  xmin=-21.25, xmax=6.25, ymin=2, ymax=28, tick style={draw=none}, xtick={-20,-15,-10,-5,0,5},
  ytick={3,7,11,15,19,23,27}, xticklabel style={font=\tiny, inner sep=1pt}, yticklabel style={font=\tiny, inner sep=1pt},
  xlabel={SNR [dB]}, ylabel={MCS index}, label style={font=\tiny}, xlabel style={yshift=0.9ex},
  title style={font=\scriptsize, yshift=-1.0ex},
  colormap={dbl}{rgb255=(33,102,172) rgb255=(103,169,207) rgb255=(209,229,240) rgb255=(247,247,247)
  rgb255=(253,219,199) rgb255=(239,138,98) rgb255=(178,24,43)}, point meta min=-1, point meta max=1},
  linkbar/.style={colorbar, colorbar style={width=0.13cm, ytick={-1,0,1}, yticklabels={$-1$,0,1},
  yticklabel style={font=\tiny}, xshift=-0.2cm}},
  linktput/.style={wpfmplot, width=2.75cm, height=2.8cm, scale only axis, xmin=-20, xmax=5, ymin=0,
  xtick={-20,-15,-10,-5,0,5}, xlabel={SNR [dB]}, ylabel={throughput [Mbit/s]}, label style={font=\tiny},
  tick label style={font=\tiny}, xlabel style={yshift=0.9ex}, title style={font=\scriptsize, yshift=-1.0ex},
  every axis plot/.append style={line width=0.7pt, mark size=1pt}}}
%
\providecommand{\linkheatplots}[1]{%
  \addplot[matrix plot*, mesh/cols=11, point meta=explicit] table[x=x, y=y, meta=c] {figs/data/v02_link_dbler_#1.dat};
  \addplot[const plot mark mid, c2, line width=0.9pt] table[x=snr, y=bW] {figs/data/v02_link_stair_#1.dat};
  \addplot[const plot mark mid, c3, line width=0.9pt] table[x=snr, y=bL] {figs/data/v02_link_stair_#1.dat};
  \addplot[const plot mark mid, black, densely dashed, line width=0.6pt] table[x=snr, y=bP] {figs/data/v02_link_stair_#1.dat};}
%
\providecommand{\linktputplots}[1]{%
  \addplot[black, densely dashed] table[x=snr_db, y=tputP] {figs/data/v02_link_tput_#1.dat};
  \addplot[c3, mark=*] table[x=snr_db, y=tputL] {figs/data/v02_link_tput_#1.dat};
  \addplot[c2, mark=*] table[x=snr_db, y=tputW] {figs/data/v02_link_tput_#1.dat};
  \addplot[c1, densely dotted, line width=0.9pt] table[x=snr_db, y=tputSm] {figs/data/v02_link_tput_#1.dat};
  \addplot[c1, only marks, mark=square, mark size=1.4pt, mark options={line width=0.6pt}] table[x=snr_db, y=tputSd] {figs/data/v02_link_tput_#1.dat};}

